Towards End-to-End Learning for Dialog State Tracking and Management using Deep Reinforcement Learning

This paper presents an end-to-end framework for task-oriented dialog systems using a variant of Deep Recurrent Q-Networks (DRQN). The model is able to interface with a relational database and jointly learn policies for both language understanding and dialog strategy. Moreover, we propose a hybrid algorithm that combines the strength of reinforcement learning and supervised learning to achieve faster learning speed. We evaluated the proposed model on a 20 Question Game conversational game simulator. Results show that the proposed method outperforms the modular-based baseline and learns a distributed representation of the latent dialog state.

==> backups.tex <==
\begin{table}[ht!]
    \centering
    \begin{tabular}{p{0.15\textwidth}p{0.05\textwidth}p{0.05\textwidth}p{0.05\textwidth}p{0.05\textwidth}} \\ \hline
    Systems                & NLU & DST & Success & NLG \\ \hline
    \cite{wen2016network}  &&Y&&Y \\
    RL                     &&&Y&Y  \\
    Hybrid-RL                   &&Y&Y&Y \\ \hline
    \end{tabular}
    \caption{Labels required for text-based task-oriented dialog systems.}
    \label{tbl:label}
\end{table}

